Evaluating the Use of Generalized Dynamic Weighted Ordinary Least Squares for Individualized HIV Treatment Strategies

Dynamic treatment regimes (DTR) are a statistical paradigm in precision medicine which aim to optimize patient outcomes by individualizing treatments. At its simplest, a DTR may require only a single decision to be made; this special case is called an individualized treatment rule (ITR) and is often used to maximize short-term rewards. Generalized dynamic weighted ordinary least squares (G-dWOLS), a DTR estimation method that offers theoretical advantages such as double robustness of parameter estimators in the decision rules, has been recently extended to now accommodate categorical treatments. In this work, G-dWOLS is applied to longitudinal data to estimate an optimal ITR, which is demonstrated in simulations. This novel method is then applied to a population affected by HIV whereby an ITR for the administration of Interleukin 7 (IL-7) is devised to maximize the duration where the CD4 load is above a healthy threshold (500 cells/$\mu$L) while preventing the administration of unnecessary injections.

==> 4-simulations.tex <==
\section{Simulation Study}
\label{section:simulation}

We carry out a simulation study to showcase the theoretical guarantees of the G-dWOLS analysis in devising a myopic treatment regime using longitudinal data. The goal of this simulation study is twofold; firstly, as presented in \cite{wallace2015doubly}, we want to illustrate the double robustness of blip parameter estimators by conducting simulations with varying sample sizes under different specifications of the treatment-free and treatment model. Secondly, we show that the myopic formulation of the optimization problem is appropriate for longitudinal data under the assumption of no delayed treatment effects. We generate longitudinal data to mimic the evolving nature of the outcome variable and time-varying confounders on which the G-dWOLS algorithm can be applied. Intra-patient correlation due to the contribution of multiple observations to the processed data is also created in the simulated data. The presentation of simulation results is done in two parts: a summary of blip parameter estimates under different simulation designs is first depicted followed by an application of the simulated results on a ``test'' population to better understand the potential advantages of the G-dWOLS' theoretical guarantees from a practical perspective.  That is, we examine bias and variability of the parameters that together specify the estimated optimal ITR, and then evaluate the impact of that ITR on a hypothetical population of new patients.% more ``practical'' approach in understanding the theoretical guarantees of G-dWOLS.

\subsection{Data Generation Procedure}

For a summary of the data generation procedure for this simulation study, see Appendix Section A.2. We let $\mathcal{O}_{ij} = \left(\text{Sex}_{ij} \equiv \text{Sex}_i, \text{CD4}_{ij}, A_{ij}, Y_{ij}\right)$ denote the $j$th stage-specific data of individual $i$ as we generate four observations, each of which we refer as a stage, for each participant. We define $Y_j$ to be some clinical outcome to be maximized and $A_j \in \{\text{0, 1, 2}\}$ to be a categorical exposure or treatment variable. Two covariates are defined: $\text{Sex}_{i}$, a time-invariant binary variable which denote a person's biological sex, and $\text{CD4}_{ij}$, a continuous time-varying variable which can represent a person's evolving CD4 cell count. Each individual is associated with four observations $\mathcal{O}_{\cdot j}$, as if these measurements were taken at each stage in a longitudinal study. The Sex variable is sampled from a Bernoulli distribution with $p =$ 0.7 whereas the CD4 variable is sampled from a truncated normal distribution denoted by $\text{TRN}_{[50, 550]}\left(350, 100\right)$ (centered around 350 with standard deviation 100 whose domain is bounded by 50 from below and 550 from above). The distribution parameters were chosen either be representative of ``real life'' or ideal in illustrating the theoretical properties of G-dWOLS; treatment effects and qualitative visualization of simulation results can vary depending on the specified model parameters. For instance, when parameter estimates are theoretically biased, the variation in CD4 counts needs to be somewhat substantial such that the bias is visually evident. The proportion of males in participants from INSPIRE studies 2 and 3 is around 70\%, hence the $p$ was specified to be 0.7 in the distribution of the Sex variable. The upper bound value of the truncated normal distribution was selected for context completeness because, in the INSPIRE protocol, patients are only eligible for treatment if their measured CD4 load is below 550 cells$/\mu$L. On the other hand, CD4 count is a strictly positive quantity and a lower bound of 50 cells$/\mu$L was chosen to reflect a lower limit of detection for testing. Treatment allocation probabilities $p_0$, $p_1$ and $p_2$ depend on parameters $\alphabf_1$ and $\alphabf_2$, which were chosen such that a reasonable proportion of generated ``people'' are assigned to each treatment category. The outputs from Algorithm~\ref{simulation} will serve as inputs for the G-dWOLS estimation procedure which was provided in more detail in section~\ref{subsection:dwols}. The assigned stage-specific treatment is sampled from a multinomial distribution whereby the probabilities $p_0,$ $p_1$ and $p_2$ for treatment allocation are defined such that they can be estimated using a logistic regression model:
\begin{align*}
    p_0 &= \frac{1}{1 + \Xbf^\alpha \alphabf_1 + \Xbf^\alpha \alphabf_2}\text{ , and}\\
    p_{\ell} &= \frac{\Xbf^\alpha \alphabf_{\ell}}{1 + \Xbf^\alpha \alphabf_1 + \Xbf^\alpha \alphabf_2} \quad \text{for } \ell = 1, 2 \, .
\end{align*}
where $X_{ij}^\alpha = \left(1, \text{Sex}_{ij}, \text{CD4}_{ij}\right)$. Although the probabilities of receiving assigned treatment $a_0,$ $a_1$ or $a_2$ are in fact covariate dependent, the indices $i$ and $j$ are dropped to alleviate the notation. We define our outcome variable $Y_{ij}$ as followed:

\begin{align*}
    Y_{ij} = X_{ij}^\beta \betabf + \one_{A_{ij} = 1}X_{ij}^\psi \psibf_1 + \one_{A_{ij} = 2}X_{ij}^\psi \psibf_2 + b_i + \epsilon_{ij}
\end{align*}

\noindent where $X_{ij}^\beta = \left(1, \exp\left\{ \text{CD4}_{ij}/200\right\}, \sqrt{\text{CD4}_{ij}} \right)$ and $X_{ij}^\psi = \left(1, \text{Sex}_{ij}, \text{CD4}_{ij}\right)$. Intra-subject correlation is generated by a time-invariant random effect $b_i$ sampled from a normal distribution centered at zero with standard deviation 0.5 and a random effect $\epsilon_{ij}$ was sampled from a $\mathcal{N}(0, 3)$ distribution. In a first simulation study, parameters were chosen to be: $\alphabf_1 =$ (-0.5, -0.2, 0.005), $\alphabf_2 =$ (-1, -0.4, 0.007), $\betabf =$ (45, -10, 1), $\psibf_1$ = (-10, 5, 0.02) and $\psibf_2 =$ (-30, -7, 0.1). The simulations are also conducted under the null, where there is no difference in expected utilities across all treatment categories. In other words, a second set of simulations is also performed with $\psibf_1 = \psibf_2 =$ (0, 0, 0) and same values for $\alphabf_1, \alphabf_2$ and $\betabf$ as in the first simulation.

\subsection{Estimation Under Various Model Specifications}

While parameters for the generalized propensity score, the treatment-free and blip models are all estimated in the G-dWOLS algorithm, interest predominantly lies in the blip coefficient estimates $\psibf$ as they provide information on the expected difference in utilities compared to baseline treatment $A =$ 0. The specification of the set of covariates on which outcome regression and estimation of generalized propensity score are performed will dictate the asymptotic behaviour of $\widehat{\psibf}$ estimates. Recall that, in G-dWOLS, the double robustness property allows misspecification of at most one of the nuisance models to ensure consistency of blip parameter estimators.
\begin{itemize}
    \item Model 1 (both treatment model and treatment-free model incorrectly specified):
    \begin{itemize}
        \item Regress $Y$ on 1, Sex, CD4 and treatments, with interactions between treatments and each of the two covariates.
        \item Fit an intercept only multinomial logistic regression\footnote{An intercept only multinomial logistic regression model does not estimate $P(A = a \, | \, \Xbf^\alpha)$ for each value of $\Xbf^\alpha$ but rather a marginal or unconditional probability, i.e.~$P(A = a \, | \, \Xbf^\alpha) = P(A = a) = n^{-1}\big(\sum_{i=1}^n \one_{A_i = a} \big)$.}.
    \end{itemize}
    \item Model 2 (correct treatment model, incorrect treatment-free model):
    \begin{itemize}
        \item Regress $Y$ on 1, Sex, CD4 and treatments, with interactions between treatments and each of the two covariates.
        \item Fit a multinomial logistic regression on 1, Sex, CD4.
    \end{itemize}
    \item Model 3 (incorrect treatment model, correct treatment-free model):
    \begin{itemize}
        \item Regress $Y$ on 1, $\exp\left\{\text{CD4/200}\right\}$, $\sqrt{\text{CD4}}$ and treatments, with interactions between treatments and each of the two covariate, where the interaction between treatment and CD4 is on the untransformed, linear CD4 scale.
        \item Fit an intercept only multinomial logistic regression.
    \end{itemize}
    \item Model 4 (both models correctly specified):
    \begin{itemize}
        \item Regress $Y$ on 1, $\exp\left\{\text{CD4/200}\right\}$, $\sqrt{\text{CD4}}$ and treatments, with interactions between treatments and each of the two covariates, where the interaction between treatment and CD4 is on the untransformed, linear CD4 scale.
        \item Fit a multinomial logistic regression on 1, Sex, CD4.
    \end{itemize}
\end{itemize}
Even though correlation was included in the data generation procedure to induce bias caused by repeated measurements, an independence correlation structure will be used in the G-dWOLS estimation process within the GEE framework. A correct specification of the covariance structure would yield more efficient estimators, but one of the main benefits of the GEE framework in accommodating longitudinal data is its asymptotic unbiasedness of linear estimates \cite{diggle2002analysis}. The standard error estimation can be done via using the sandwich estimator or bootstrapping, but we used the former method to alleviate computational burden.\b

The simulation study was conducted on sample sizes $n =$ 100 and $n =$ 1000 to investigate sample properties of estimators. As mentioned in section~\ref{subsection:dwols}, IPT and overlap weights both satisfy the balancing property, a feature of the dWOLS algorithm that ensures the double robustness of $\widehat{\psibf}$; both weights were used in analyzing the simulated data. Each simulation design requires a choice of sample size $n$, G-dWOLS weight function (IPT or overlap) and one of four possible model specifications. To numerically assess the underlying properties of our statistical methodology, 1000 Monte Carlo replications were carried out for all possible simulation scenario combinations.

\subsection{Simulation Results}
\label{subsection:simulation-results}

The presentation of the results from the simulation study will be split into two parts: a summary of blip coefficient estimates followed by an application of these estimates on a completely novel or ``test'' set of 10 000 subject-level data. In a first instance, an overview of the variation and median of the $\widehat{\psibf}$ estimated values across the $1000$ replications would provide a better idea on the effects of sample sizes, weight function choice and model specification on the blip coefficient estimates. Afterwards, the application of simulation results on an out-of-sample population would shed light on the quantitative benefits of the G-dWOLS estimation procedure in tailoring treatment to individual-level information.

\subsubsection{Summary of Blip Coefficient Estimates}
\label{subsection:summary-simulations}
% Note that this example is extendable to cases with more than $3$ treatment categories and more than $4$ treatment stages.

Each point estimate of $\psibf$ is obtained by applying the G-dWOLS algorithm on a generated dataset consisting of $n$ subjects, for $n =$ 100 or $n =$ 1000 as mentioned previously. The results of the simulation study are showcased in Figures~\ref{fig:simulation-1} and~\ref{fig:simulation-null}, which display boxplots summarizing the estimates across the 1000 runs for the non-null and null simulation settings. For purposes of notational simplicity, $\psi_{\cdot 1}$ is the blip model coefficient for Sex whereas $\psi_{\cdot 2}$ is that for CD4, with the $\cdot$ representing treatment level 1 or 2, relative to baseline level of treatment. Because similar conclusions can be drawn from the numerical results presented in both figures, the focus of this discussion will be on Figure~\ref{fig:simulation-1}.
\begin{figure*}[!htp]
    \centering
    \includegraphics[width=\textwidth]{simulation-plots/simulation-results.png}
    \caption[Boxplots of $\widehat{\psibf}$ estimates under different simulation designs.]{Boxplots of $\widehat{\psibf}$ estimates are displayed for four different model specifications, for two different sample sizes ($n =$ 100, 1000) and for two forms of balancing weights (IPT and overlap). The top row corresponds to the blip parameters for treatment level 1 (relative to level 0) and the bottom row to treatment level 2. The first column represents the main effect of treatment level, the middle and right columns are, respectively, the interactions of treatment with Sex and CD4.}
    \label{fig:simulation-1}
    \includegraphics[width=\textwidth]{simulation-plots/simulation-results_null.png}
    \caption[Boxplots of $\widehat{\psibf}$ estimates under different simulation designs and no treatment effect.]{Boxplots of $\widehat{\psibf}$ estimates are displayed for four different model specifications, for two different sample sizes and for two forms of balancing weights whereby all blip parameters set to 0 in the data generating process. Rows and columns are as in Figure~\ref{fig:simulation-1}.}
    \label{fig:simulation-null}
\end{figure*}

The first row is parameters corresponding to treatment $A =$ 1 whereas the second row corresponds to treatment $A =$ 2. In each plot, there are boxplots grouped with respect to the four different combinations of model specifications as described on the previous page (Models 1, 2, 3 and 4). Labelled by their shading and hatch pattern, each set itself showcases the simulation results under different sample sizes and G-dWOLS weight form. The dotted horizontal line in every plot indicates the true value of the parameter used in the data generating process. The most important visual pattern across the plots is the bias of estimated values under Model 1. This result is not surprising, as G-dWOLS does not guarantee consistency when both nuisance models are incorrectly specified. However, it is important to point out that the estimates of $\psi_{11}$ and $\psi_{21}$ under Model 1 do not depart significantly from the true parameter value. In other words, unbiasedness can still be achieved but it is not guaranteed in Model 1. Other noticeable patterns are the decreasing interquartile range from $n =$ 100 to $n =$ 1000, which is evidence of a gain in efficiency with increasing sample size. The relative closeness between the median of estimates in Models 2, 3 and 4 and the true parameter values depicted by horizontal dotted lines suggests that unbiasedness can be reached in reasonable sample sizes. Although the simulation results show that finite sample performance improves with increasing values of $n$, $\psibf$ estimates at $n =$ 100 perform well and data analysis results using similar sample sizes can yield good point estimates with reasonable variability provided that researchers are confident in the modelling choices. The difference in using IPT weights and overlap weights, which can be inferred by comparing boxplots with diagonal hatch patterns to the ones without such patterns, does not seem to be dramatic. That being said, the smaller variability in $\widehat{\psibf}$ estimates when using overlap weights suggest that having them bounded between 0 and 1 provide a more precise point estimate, since IPT weights are unbounded from above \cite{wallace2015doubly}.% This conclusion is indicative of little difference in the analysis between the two possible G-dWOLS weight specifications. As such, the data analysis in section~\ref{section:results} can be carried out with either IPT weights or overlap weights; IPT weights were primarily for convenience purposes.

\subsubsection{Average Utilities and Agreement Rates}

A collection of data comprised of out-of-sample 10 000 subjects, which have not been used in the estimating process, is generated using Algorithm~\ref{simulation} as well to further examine and validate the results of the simulation study. Since this additional dataset was not used in obtaining estimates of blip function parameters, two comparisons which stem from this newly created set of potential participants are made. Firstly, the expected outcome value under uniform treatment (e.g.~all 10 000 ``test'' people receive medical intervention $A =$ 0, 1 or 2) are evaluated. Secondly, the utility under the estimated optimal treatment denoted by $\widehat{A}^{\opt}$ depends on the value of $\widehat{\psibf}$ of a given iteration. The estimated ideal treatment $\widehat{A}^\opt$ in patient-stages will be compared to the true values of $A^\opt$, whereby the proportion of $A^\opt$ agreeing with $\widehat{A}^\opt$ will be referred to as the agreement rate. In Figure~\ref{fig:simulation-2}, we show the average outcome value under $\widehat{A}^{\opt}$ for the out-of-sample data which we define as $\overline{Y}^{\opt} = \sum_{i=1}^{10\,000} \E[Y \, | \, \Xbf=\xbf_i,\, A = \widehat{A}^{\opt}; \widehat{\psibf}]$. Note that the true values of $A^\opt$ are known for all patient-stages since blip coefficient parameters are known by design in a simulation study, fixed by the choice of data-generating parameters.

\begin{figure}[!htp]
    \centering
    \includegraphics[width=\textwidth]{simulation-plots/average-utility-under-estimated-optimal-treatment.png}
    \caption[Average outcome under different simulation designs.]{Average outcome under different model specifications using blip coefficients estimated with different sample sizes; the corresponding agreement rate is displayed on top of each bar. Dotted lines are the average utilities under uniform treatment, labelled respectively by the treatment options $A =$ 0, 1 or 2; average utility under optimal treatment is indicated by $A^{\opt}$.}
    \label{fig:simulation-2}
\end{figure}

In the absence of substantial variability in the outcome variable or treatment effects, a perfect agreement rate can be attained in drawing meaningful conclusions regarding the effect of sample size, forms of G-dWOLS weight functions and model specifications on the estimation of optimal treatment. The values of $\overline{Y}^{\opt}$ are represented by the height of each bar in Figure~\ref{fig:simulation-2} for various model specifications. The corresponding agreement rate for each simulation design is displayed on top of the bars in the barplot. Results confirm that the selection of weight function for the G-dWOLS algorithm provides comparable results, although the overlap weights seem slightly better in Model 2 where only the treatment is correctly specified. Models 2, 3 and 4 show that larger outcome values and better agreement rates can be achieved in light of the correct specification of at least one of the treatment-free or treatment model. However, for $n =$ 100, Model 3 and 4 seem to outperform Model 2, which suggests that the gain in efficiency can be slightly different in smaller sample sizes depending on which nuisance model is correctly specified. Nonetheless, the main conclusion that can be extracted from Figures~\ref{fig:simulation-1} and~\ref{fig:simulation-2} is that desirable results are achievable in relatively larger sample sizes given that at least one of the nuisance models is correctly specified and the chosen weight function adheres to the balancing property.
